FOOL: Addressing the Downlink Bottleneck in Satellite Computing with Neural Feature Compression

Nanosatellite constellations equipped with sensors capturing large geographic regions provide unprecedented opportunities for Earth observation. As constellation sizes increase, network contention poses a downlink bottleneck. Orbital Edge Computing (OEC) leverages limited onboard compute resources to reduce transfer costs by processing the raw captures at the source. However, current solutions have limited practicability due to reliance on crude filtering methods or over-prioritizing particular downstream tasks. This work presents FOOL, an OEC-native and task-agnostic feature compression method that preserves prediction performance. FOOL partitions high-resolution satellite imagery to maximize throughput. Further, it embeds context and leverages inter-tile dependencies to lower transfer costs with negligible overhead. While FOOL is a feature compressor, it can recover images with competitive scores on quality measures at lower bitrates. We extensively evaluate transfer cost reduction by including the peculiarity of intermittently available network connections in low earth orbit. Lastly, we test the feasibility of our system for standardized nanosatellite form factors. We demonstrate that FOOL permits downlinking over 100x the data volume without relying on prior information on the downstream tasks.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> embed/equations/pixels_per_seconds.tex <==
%\begin{equation}
%\frac{\text { Batch Size } \times \text { %Image Height } \times \text { Image Width } %\times \text { Bands }}{\text { Seconds per %Batch }}    
%\end{equation}

\begin{equation}
\text{PP/s} = \frac{B \times H \times W \times C}{\text{Seconds per Batch}}
\end{equation}


==> embed/equations/transfer_cost_reduced_per_seconds_log.tex <==
\begin{equation}
\text{TCR/s} = \underbrace{\frac{B \times H \times W \times C}{\text{Seconds per Batch}}}_{\text{PP/s}} \times 
%\left(
\frac{\operatorname{log}(\text{bpp}_{\text{raw}})}{ \operatorname{log}(\text{bpp}_{\text{enc}})}
%\right)
\label{eq:tcrs}  
\end{equation}


==> embed/media/fig_fool_detection_pipeline.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/fool-hlvl-split-pt2-v3.pdf}
    \caption{Detection Pipeline for Evaluation}
    \label{fig:detectionpipeline}
\end{figure}

==> embed/media/fig_fool_hlvl.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/fool-hlvl.pdf}
    \caption{Prediction High Level Overview}
    \label{fig:foolhlvl}
\end{figure}

==> embed/media/fig_framework.tex <==
% TODO: Remove from here
% !TeX root = main.tex

\begin{figure}[t]
	\centering
%	\begin{minipage}[b]{0.23\textwidth}
%		\includegraphics[width=1\textwidth]{figs/live-streaming-buffer}
%		\subcaption{Jitter buffer size}
%	\end{minipage}
%	~
	\begin{minipage}[b]{0.48\textwidth}
		\includegraphics[width=1\textwidth]{figures/ecosystem.pdf}
		%\subcaption{Network and transcoding}
	\end{minipage}
	
	\caption{The service framework of existing EO ecosystems.}
	
	\label{fig:ecosystem}
	\vspace{-15pt}
\end{figure}

==> embed/media/fig_leftoverdep_vs_keypoints.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/aerials_kps_vs_leftover2row.png}
    \caption{Leftover Dependencies (middle), Keypoints (right)}
    \label{fig:leftovervskeypoints}
\end{figure}

==> embed/media/fig_mult_backbones_mult_tasks.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/mult-backbones-mult-tasks.pdf}
    \caption{Multiple Backbones with Multiple Tasks}
    \label{fig:multbbmulttasks}
\end{figure}

==> embed/media/fig_seq_vs_par.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/seq-vs-par-exec.pdf}
    \caption{Sequential and Parallelizable Execution of DNNs}
    \label{fig:seqvsparexec}
\end{figure}

==> embed/media/fig_tensor_reshaping.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/reshaping-tensors.pdf}
    \caption{Reshaping and Permuting Image Tensors}
    \label{fig:tensorreshape}
\end{figure}

==> embed/tables/backbone-overview.tex <==
\begin{table}[htb]
\centering
\caption{Client Detection Model Architectures and Tasks }
\label{tab:backboneperformance}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccc}
\hline
Model                      & Task                               & mAP@50                       & mAP@50:95                    \\ \hline
                           & DOTA-2                             & 53.1                         & 33.1                         \\
                           & \cellcolor[HTML]{EFEFEF}SpaceNet-3 & \cellcolor[HTML]{EFEFEF}37.5 & \cellcolor[HTML]{EFEFEF}20.5 \\
\multirow{-3}{*}{YOLOv8-M} & xView                              & 38.2                         & 20.8                         \\ \hline
                           & \cellcolor[HTML]{EFEFEF}DOTA-2     & \cellcolor[HTML]{EFEFEF}53.1 & \cellcolor[HTML]{EFEFEF}33.1 \\
                           & SpaceNet-3                         & 37.5                         & 20.5                         \\
\multirow{-3}{*}{YOLOv8-L} & \cellcolor[HTML]{EFEFEF}xView      & \cellcolor[HTML]{EFEFEF}38.2 & \cellcolor[HTML]{EFEFEF}20.8 \\ \hline
                           & DOTA-2                             & 53.1                         & 33.1                         \\
                           & \cellcolor[HTML]{EFEFEF}SpaceNet-3 & \cellcolor[HTML]{EFEFEF}37.5 & \cellcolor[HTML]{EFEFEF}20.5 \\
\multirow{-3}{*}{YOLOv5-M} & xView                              & 38.2                         & 20.8                         \\
                           & \cellcolor[HTML]{EFEFEF}DOTA-2     & \cellcolor[HTML]{EFEFEF}53.1 & \cellcolor[HTML]{EFEFEF}33.1 \\
                           & SpaceNet-3                         & 37.5                         & 20.5                         \\
\multirow{-3}{*}{YOLOv5-M} & \cellcolor[HTML]{EFEFEF}xView      & \cellcolor[HTML]{EFEFEF}38.2 & \cellcolor[HTML]{EFEFEF}20.8
\end{tabular}%
}
\end{table}

==> embed/tables/comp_throughput_no_concurrent.tex <==
\begin{table}[htb]
\caption{Throughput Comparison Between Feature Codecs}
\label{tab:sumcompthroughput}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
Model &
  \begin{tabular}[c]{@{}c@{}}PP/s \\ (Orin Nano)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}PP/s\\ (NX)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}PP/s\\ (TX2)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}PC/s \\ (Orin Nano)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}PC/s\\ (NX)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}PC/s\\ (TX2)\end{tabular} \\ \hline
\rowcolor[HTML]{EFEFEF} 
FOOL-L     & TBD & TBD & TBD & TBD & TBD & TBD \\
FOOL-M     & TBD & TBD & TBD & TBD & TBD & TBD \\
\rowcolor[HTML]{EFEFEF} 
FOOL-S     & TBD & TBD & TBD & TBD & TBD & TBD \\ \hline
Ablation-L & TBD & TBD & TBD & TBD & TBD & TBD \\
\rowcolor[HTML]{EFEFEF} 
Ablation-M & TBD & TBD & TBD & TBD & TBD & TBD \\
Ablation-S & TBD & TBD & TBD & TBD & TBD & TBD \\ \hline
\rowcolor[HTML]{EFEFEF} 
BSVBI-L    & TBD & TBD & TBD & TBD & TBD & TBD \\
BSVBI-M    & TBD & TBD & TBD & TBD & TBD & TBD \\
\rowcolor[HTML]{EFEFEF} 
BSVBI-S    & TBD & TBD & TBD & TBD & TBD & TBD \\ \hline
\end{tabular}%
}
\end{table}

==> embed/tables/complete_pipeline_throughput.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
\caption{Throughput Evaluation of Complete Pipeline}
\label{tab:completepipeline}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\hline
Model &
  Device &
  \begin{tabular}[c]{@{}c@{}}Input Size\\ (MB)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Sequential\\ (MB/s)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Concurrent\\ (MB/s)\end{tabular} \\ \hline
                             & \cellcolor[HTML]{EFEFEF}Orin Nano & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
                             & TX2                               & 42                         & 4.2                         & 4.2                         \\
\multirow{-3}{*}{FOOL-L}     & \cellcolor[HTML]{EFEFEF}NX        & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
                             & Orin Nano                         & 42                         & 4.2                         & 4.2                         \\
                             & \cellcolor[HTML]{EFEFEF}TX2       & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
\multirow{-3}{*}{FOOL-M}     & NX                                & 42                         & 4.2                         & 4.2                         \\
                             & \cellcolor[HTML]{EFEFEF}Orin Nano & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
                             & TX2                               & 42                         & 4.2                         & 4.2                         \\
\multirow{-3}{*}{FOOL-S}     & \cellcolor[HTML]{EFEFEF}NX        & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\ \hline
                             & Orin Nano                         & 42                         & 4.2                         & 4.2                         \\
                             & \cellcolor[HTML]{EFEFEF}TX2       & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
\multirow{-3}{*}{Ablation-L} & NX                                & 42                         & 4.2                         & 4.2                         \\
                             & \cellcolor[HTML]{EFEFEF}Orin Nano & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
                             & TX2                               & 42                         & 4.2                         & 4.2                         \\
\multirow{-3}{*}{Ablation-M} &
  \cellcolor[HTML]{EFEFEF}NX &
  \cellcolor[HTML]{EFEFEF}42 &
  \cellcolor[HTML]{EFEFEF}4.2 &
  \cellcolor[HTML]{EFEFEF}4.2 \\
                             & Orin Nano                         & 42                         & 4.2                         & 4.2                         \\
                             & \cellcolor[HTML]{EFEFEF}TX2       & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
\multirow{-3}{*}{Ablation-S} & NX                                & 42                         & 4.2                         & 4.2                         \\ \hline
                             & \cellcolor[HTML]{EFEFEF}Orin Nano & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
                             & TX2                               & 42                         & 4.2                         & 4.2                         \\
\multirow{-3}{*}{BSVBI-L}    & \cellcolor[HTML]{EFEFEF}NX        & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
                             & Orin Nano                         & 42                         & 4.2                         & 4.2                         \\
                             & \cellcolor[HTML]{EFEFEF}TX2       & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
\multirow{-3}{*}{BSVBI-M}    & NX                                & 42                         & 4.2                         & 4.2                         \\
                             & \cellcolor[HTML]{EFEFEF}Orin Nano & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
                             & TX2                               & 42                         & 4.2                         & 4.2                         \\
\multirow{-3}{*}{BSVBI-S}    & \cellcolor[HTML]{EFEFEF}NX        & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\ \hline
\end{tabular}%
}
\end{table}

==> embed/tables/energy_consumption.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[htb]
\centering
\caption{Energy Usage and Savings from Rate Reduction}
\label{tab:energyconsumption}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\hline
Device & Model & Inference (J) \textdownarrow \textdownarrow & Pipeline (J) \textdownarrow \textdownarrow & T. Red. (\%) \textuparrow \textuparrow \\ \hline
                            & \cellcolor[HTML]{EFEFEF}FOOL-S & \cellcolor[HTML]{EFEFEF}TBD & \cellcolor[HTML]{EFEFEF}TBD & \cellcolor[HTML]{EFEFEF}TBD \\
\multirow{-2}{*}{Orin Nano} & BSVBI-M                        & TBD                         & TBD                         & TBD                         \\ \hline
                            & \cellcolor[HTML]{EFEFEF}FOOL-S & \cellcolor[HTML]{EFEFEF}TBD & \cellcolor[HTML]{EFEFEF}TBD & \cellcolor[HTML]{EFEFEF}TBD \\
\multirow{-2}{*}{NX}        & BSVBI-M                        & TBD                         & TBD                         & TBD                         \\ \hline
                            & \cellcolor[HTML]{EFEFEF}FOOL-S & \cellcolor[HTML]{EFEFEF}TBD & \cellcolor[HTML]{EFEFEF}TBD & \cellcolor[HTML]{EFEFEF}TBD \\
\multirow{-2}{*}{TX2}       & BSVBI-M                        & TBD                         & TBD                         & TBD                         \\ \hline
\end{tabular}%
}
\end{table}

==> embed/tables/entropycoderperf.tex <==
\begin{table}[htb]
\centering
\caption{Performance for Entropy Coding Files}
\label{tab:entropycodingfiles}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccccc}
\hline
Model &
  Device &
  Spatial Dim &
  \begin{tabular}[c]{@{}c@{}}Inference \\ (Files/s)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}File Size\\ (MB)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}rANS seq. \\ (MB/s)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}rANS w\textbackslash{}inf. \\ (MB/s)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}rANS w\textbackslash{}both. \\ (MB/s)\end{tabular} \\ \hline
 &
  \cellcolor[HTML]{EFEFEF}Orin Nano &
  \cellcolor[HTML]{EFEFEF}$500\times500$ &
  \cellcolor[HTML]{EFEFEF}4.20 &
  \cellcolor[HTML]{EFEFEF}0.420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 \\
 &
  TX2 &
  $500\times500$ &
  4.20 &
  0.420 &
  420 &
  420 &
  420 \\
\multirow{-3}{*}{FOOL-L} &
  \cellcolor[HTML]{EFEFEF}NX &
  \cellcolor[HTML]{EFEFEF}$500\times500$ &
  \cellcolor[HTML]{EFEFEF}4.20 &
  \cellcolor[HTML]{EFEFEF}0.420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 \\ \hline
 &
  Orin Nano &
  $500\times500$ &
  4.20 &
  0.420 &
  420 &
  420 &
  420 \\
 &
  \cellcolor[HTML]{EFEFEF}TX2 &
  \cellcolor[HTML]{EFEFEF}$500\times500$ &
  \cellcolor[HTML]{EFEFEF}4.20 &
  \cellcolor[HTML]{EFEFEF}0.420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 \\
\multirow{-3}{*}{FOOL-M} &
  NX &
  $500\times500$ &
  4.20 &
  0.420 &
  420 &
  420 &
  420 \\ \hline
 &
  \cellcolor[HTML]{EFEFEF}Orin Nano &
  \cellcolor[HTML]{EFEFEF}$500\times500$ &
  \cellcolor[HTML]{EFEFEF}4.20 &
  \cellcolor[HTML]{EFEFEF}0.420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 \\
 &
  TX2 &
  $500\times500$ &
  4.20 &
  0.420 &
  420 &
  420 &
  420 \\
\multirow{-3}{*}{FOOL-S} &
  \cellcolor[HTML]{EFEFEF}NX &
  \cellcolor[HTML]{EFEFEF}$500\times500$ &
  \cellcolor[HTML]{EFEFEF}4.20 &
  \cellcolor[HTML]{EFEFEF}0.420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 \\ \hline
\end{tabular}%
}
\end{table}

==> embed/tables/impact_no_tiles.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[htb]
\centering
\caption{Effect of Number of TIles on Bpp}
\label{tab:impacttiles}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{ccccc}
% \hline
\begin{tabularx}{\columnwidth}{@{\extracolsep{\fill}} 
% >{\raggedright\arraybackslash} p{0.14\linewidth} 
ccccc }
Model & Tiles & DOTA-2 (bpp \textdownarrow \textdownarrow) &
SpaceNet-3 (bpp \textdownarrow \textdownarrow) & xView (bpp \textdownarrow \textdownarrow) \\ \hline
& \cellcolor[HTML]{EFEFEF}3 & \cellcolor[HTML]{EFEFEF}0.2029 & \cellcolor[HTML]{EFEFEF}0.1931 & \cellcolor[HTML]{EFEFEF}0.1983 \\
& 4                         & 0.1918                         & 0.1863                         & 0.1886     \\
\multirow{-3}{*}{FOOL-L} &
  \cellcolor[HTML]{EFEFEF}5 &
  \cellcolor[HTML]{EFEFEF}\textbf{0.1843} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.176} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.1822} \\ \hline
                         & 3                         & 0.2205                         & 0.2188                         & 0.2203                         \\
                         & \cellcolor[HTML]{EFEFEF}4 & \cellcolor[HTML]{EFEFEF}0.2148 & \cellcolor[HTML]{EFEFEF}0.2079 & \cellcolor[HTML]{EFEFEF}0.2125 \\
\multirow{-3}{*}{FOOL-M} & 5                         & \textbf{0.2093}                & \textbf{0.201}                 & \textbf{0.2072}                \\ \hline
                         & \cellcolor[HTML]{EFEFEF}3 & \cellcolor[HTML]{EFEFEF}0.2501 & \cellcolor[HTML]{EFEFEF}0.420  & \cellcolor[HTML]{EFEFEF}0.420  \\
                         & 4                         & 0.2490                         & 0.420                          & 0.420                          \\
\multirow{-3}{*}{FOOL-S} &
  \cellcolor[HTML]{EFEFEF}5 &
  \cellcolor[HTML]{EFEFEF}\textbf{0.2468} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.2385} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.2447} \\ \hline
\end{tabularx}%
% }
\end{table}

==> embed/tables/optim_config_memory.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\hline
Model                                                                                     & Device                            & Spatial Dims                    & Tiles                     & Memory (MB)                    \\ \hline
                                                                                          & \cellcolor[HTML]{EFEFEF}Orin Nano & \cellcolor[HTML]{EFEFEF}500x500 & \cellcolor[HTML]{EFEFEF}5 & \cellcolor[HTML]{EFEFEF}24,000 \\
                                                                                          & TX                                & 500x500                         & 5                         & 24,000                         \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}\{FOOL,\\ Ablation,\\ BSVBI\}-L\end{tabular}} & \cellcolor[HTML]{EFEFEF}NX2       & \cellcolor[HTML]{EFEFEF}500x500 & \cellcolor[HTML]{EFEFEF}5 & \cellcolor[HTML]{EFEFEF}24,000 \\ \hline
                                                                                          & Orin Nano                         & 500x500                         & 5                         & 24,000                         \\
                                                                                          & \cellcolor[HTML]{EFEFEF}TX        & \cellcolor[HTML]{EFEFEF}500x500 & \cellcolor[HTML]{EFEFEF}5 & \cellcolor[HTML]{EFEFEF}24,000 \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}\{FOOL,\\ Ablation,\\ BSVBI\}-M\end{tabular}} & NX2                               & 500x500                         & 5                         & 24,000                         \\ \hline
                                                                                          & \cellcolor[HTML]{EFEFEF}Orin Nano & \cellcolor[HTML]{EFEFEF}500x500 & \cellcolor[HTML]{EFEFEF}5 & \cellcolor[HTML]{EFEFEF}24,000 \\
                                                                                          & TX                                & 500x500                         & 5                         & 24,000                         \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}\{FOOL,\\ Ablation,\\ BSVBI\}-S\end{tabular}} & \cellcolor[HTML]{EFEFEF}NX2       & \cellcolor[HTML]{EFEFEF}500x500 & \cellcolor[HTML]{EFEFEF}5 & \cellcolor[HTML]{EFEFEF}24,000 \\ \hline
\end{tabular}%
}
\caption{Configurations That Maximize Throughput}
\label{tab:optimconfigmemory}
\end{table}
